Attack as the Best Defense: Nullifying Image-to-image Translation GANs via Limit-aware Adversarial Attack

With the successful creation of high-quality image-to-image (Img2Img) translation GANs comes the non-ethical applications of DeepFake and DeepNude. Such misuses of img2img techniques present a challenging problem for society. In this work, we tackle the problem by introducing the Limit-Aware Self-Guiding Gradient Sliding Attack (LaS-GSA). LaS-GSA follows the Nullifying Attack to cancel the img2img translation process under a black-box setting. In other words, by processing input images with the proposed LaS-GSA before publishing, any targeted img2img GANs can be nullified, preventing the model from maliciously manipulating the images. To improve efficiency, we introduce the limit-aware random gradient-free estimation and the gradient sliding mechanism to estimate the gradient that adheres to the adversarial limit, i.e., the pixel value limitations of the adversarial example. Theoretical justifications validate how the above techniques prevent inefficiency caused by the adversarial limit in both the direction and the step length. Furthermore, an effective self-guiding prior is extracted solely from the threat model and the target image to efficiently leverage the prior information and guide the gradient estimation process. Extensive experiments demonstrate that LaS-GSA requires fewer queries to nullify the image translation process with higher success rates than 4 state-of-the-art black-box methods.

==> thefigs/app_ext_ablation.tex <==
\begin{table*}\small
    \caption{The quantitative results of the distorting attack and the nullifying attack adding S-RGF for the ablation study.}
    \centering
    \vspace{1mm}
    \begin{tabular}{|c|cc|cc|cc|}
    \multicolumn{7}{c}{\textbf{Distorting Attack}} \\
    \hline
        \multirow{2}{*}{Methods}
        & \multicolumn{2}{|c|}{\textsc{street2segment} (1)}
        & \multicolumn{2}{|c|}{\textsc{facade2label} (1)}
        & \multicolumn{2}{|c|}{\textsc{label2facade} (1)} \\
        \cline{2-7}
        & ASR & AVG. Q & ASR & AVG. Q & ASR & AVG. Q \\
    \hline
        RGF & 94.8\% & 26,343 & 94.7 \% & 30,452 & 51.3\% &  51,452  \\
        P-RGF & 95.1\% & \textbf{17,719}  & 90.3\% & \textbf{24,378}   & 44.2\% & 56,575  \\  
        \hline
        S-RGF & 90.0\% & 19,453  & 95\% & 30,400   & 50\% & 57,760  \\  
        LaS-RGF & \textbf{100.0\%} & 21,631 & \textbf{100.0\%} & 26,405 & \textbf{79.3\%} & \textbf{47,080}  \\  
    \hline
    \end{tabular}

    \centering
    \vspace{1mm}
    \begin{tabular}{|c|cc|cc|cc|}
   
    \multicolumn{7}{c}{\textbf{Nullifying Attack}}\\
    \hline
        \multirow{2}{*}{Methods}
        & \multicolumn{2}{|c|}{\textsc{black2blond} (0.9)}
        & \multicolumn{2}{|c|}{\textsc{horse2zebra} (0.5)}
        & \multicolumn{2}{|c|}{\textsc{photo2paint} (0.8)} \\
        \cline{2-7}
        & ASR & AVG. Q & ASR & AVG. Q & ASR & AVG. Q \\
    \hline
        RGF & 25.2\% & 54,455 & 60.4\% & 40,207 & 64.3\% & \textbf{37,422}\\
        P-RGF & 25.1\% & 52,601 & 55.2\% & 34,439    & 64.4\% &  38,925\\
        \hline
        S-RGF & 25.0\% & 52,652 & 60.0\% & 41,375  & \textbf{70.0\%} &  51,572\\
        LaS-RGF  & \textbf{80.9\%} & \textbf{38,706} & \textbf{75.7\%} & \textbf{16,885} & 62.9\% & 42,126 \\  
    \hline
    \end{tabular}
    \label{ap-table:ablation}
    \vspace{-2mm}
\end{table*}


==> thefigs/app_ext_compare_classify.tex <==
\begin{table}
    \caption{Comparing the results of P-RGF and the incorporation of limit-aware RGF to the P-RGF method (LaP-RGF).}
    \centering
    \vspace{1mm}
    \begin{tabular}{|c|cc|cc|cc|}
    \hline
        \multirow{2}{*}{Methods}
        & \multicolumn{2}{|c|}{Inception-v3}
        & \multicolumn{2}{|c|}{VGG-16}
        & \multicolumn{2}{|c|}{ResNet-50} \\
        \cline{2-7}
        & ASR & Q & ASR & Q & ASR & Q \\
    \hline
        P-RGF&  90.9\%&\textbf{638}&     93.4\%&329      &94.7\%&\textbf{454}\\  
        \hline
        LaP-RGF& \textbf{91.8\%} &678&    \textbf{93.5\%}&\textbf{301}      &\textbf{97.4\%}&552\\  
    \hline
    \end{tabular}
    \label{tab:classify}
\end{table}


==> thefigs/app_ext_limits.tex <==
\begin{figure*}[t]\small
    \centering
        \begin{subfigure}{.95\linewidth}
            \centering
    		\includegraphics[width=0.98\linewidth]{theimgs/app_ext_plots/lab2face_limitplot.jpg}
            \caption{{\scriptsize\textsc{label2facade}}}
    	\end{subfigure}
        \begin{subfigure}{.95\linewidth}
            \centering
    		\includegraphics[width=0.98\linewidth]{theimgs/app_ext_plots/blond_limitplot.jpg}
            \caption{{\scriptsize\textsc{black2blond}}}
    	\end{subfigure}
        \caption{The distortion score ($s_{Dist}$) of \textsc{label2facade} and the nullifying score ($s_{Null}$) of \textsc{black2blond} with different $\epsilon$.}
    \label{fig:limitscore}
\end{figure*}

%  Red, blue, green lines denote \modelNameShort, P-RGF, RGF, and solid line, dotted line, ``x'' markers, and ``+'' markers denote $\epsilon=1, 0.07, 0.04, 0.01$ respectively.



==> thefigs/app_ext_query.tex <==
\begin{figure*}[t]\small
    \centering
        \begin{subfigure}{.95\linewidth}
            \centering
    		\includegraphics[width=0.98\linewidth]{theimgs/app_ext_plots/lab2face_mrlsplot.jpg}
            \caption{{\scriptsize\textsc{label2facade}}}
    	\end{subfigure}
        \begin{subfigure}{.95\linewidth}
            \centering
    		\includegraphics[width=0.98\linewidth]{theimgs/app_ext_plots/blond_mrlsplot.jpg}
            \caption{{\scriptsize\textsc{black2blond}}}
    	\end{subfigure}
        \caption{The distortion score ($s_{Dist}$) of \textsc{label2facade} and the nullifying score ($s_{Null}$) of \textsc{black2blond} with different $q$.}
    \label{fig:queryscore}
\end{figure*}


==> thefigs/app_final_visuals/all_stack_dist.tex <==
\begin{figure*}[t]
\captionsetup[subfigure]{labelformat=empty}
    \centering
    
    %str2seg
    
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/str2seg/9-x0.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/str2seg/9-y0.jpg}
        \caption{original}
	\end{subfigure}
    \centering
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/str2seg/x-0.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/str2seg/y-0-83-1056.jpg}
        \caption{$0.83-1056$}
	\end{subfigure}
    \begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/str2seg/x-3.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/str2seg/y-3-131-4221.jpg}
        \caption{$1.31-4221$}
	\end{subfigure}
    \begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/str2seg/x-12.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/str2seg/y-12-171-13716.jpg}
        \caption{$1.71-13716$}
	\end{subfigure}
    \begin{subfigure}{.16\linewidth}
            \centering
            \includegraphics[width=.98\linewidth]{theimgs/app_final_process/str2seg/x-45.jpg}
            \includegraphics[width=.98\linewidth]{theimgs/app_final_process/str2seg/y-45-220-48531.jpg}
            \caption{$2.2-48531$}
    	\end{subfigure}
    \begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/str2seg/x-93.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/str2seg/y-93-265-99171.jpg}
        \caption{$2.65-99171$}
	\end{subfigure}
	
	% facade2label
	
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/faca2lab/2-x0.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/faca2lab/2-y0.jpg}
        \caption{original}
	\end{subfigure}
    \centering
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/faca2lab/x-0.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/faca2lab/y-0-21-1055.jpg}
        \caption{$0.21-1055$}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/faca2lab/x-2.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/faca2lab/y-2-47-3163.jpg}
        \caption{$0.47-3163$}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/faca2lab/x-8.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/faca2lab/y-8-75-9487.jpg}
        \caption{$0.75-9487$}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/faca2lab/x-19.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/faca2lab/y-19-101-21081.jpg}
        \caption{$1.01-21081$}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/faca2lab/x-93.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/faca2lab/y-93-126-99077.jpg}
        \caption{$1.26-99077$}
	\end{subfigure}

	%label2facade
	
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/lab2face/0-x0.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/lab2face/0-y0.jpg}
        \caption{original}
	\end{subfigure}
    \centering
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/lab2face/x-0.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/lab2face/y-0-23-1056.jpg}
        \caption{$0.23-1055$}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/lab2face/x-5.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/lab2face/y-5-53-6331.jpg}
        \caption{$0.53-6311$}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/lab2face/x-11.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/lab2face/y-11-81-12661.jpg}
        \caption{$0.81-12661$}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/lab2face/x-25.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/lab2face/y-25-112-27431.jpg}
        \caption{$1.12-27431$}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/lab2face/x-82.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/lab2face/y-82-140-87566.jpg}
        \caption{$1.40-87566$}
	\end{subfigure}
	
    \caption{The illustrations of \modelNameShort applied to the distorting attack process on \textsc{street2segment}, \textsc{facade2label} and \textsc{label2facade}.}
    \label{fig:process-dist}
    \end{figure*}
    


	


==> thefigs/app_final_visuals/all_stack_null.tex <==
\begin{figure*}[t]
\captionsetup[subfigure]{labelformat=empty}
    \centering
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/blond/16.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/blond/16a.jpg}
        \caption{original}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/blond/x-0.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/blond/y-0-40-1056.jpg}
        \caption{$0.40-1056$}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/blond/x-5.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/blond/y-5-54-6331.jpg}
        \caption{$0.54-6331$}
	\end{subfigure}
		\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/blond/x-9.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/blond/y-9-67-10551.jpg}
        \caption{$0.67-10551$}
	\end{subfigure}
		\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/blond/x-29.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/blond/y-29-78-31651.jpg}
        \caption{$0.78-31651$}
	\end{subfigure}
		\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/blond/x-91.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/blond/y-91-94-97061.jpg}
        \caption{$0.94-97061$}
	\end{subfigure}
	
	
	
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/horse/15-x0.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/horse/15-y0.jpg}
        \caption{original}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/horse/x-3.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/horse/y-3-14-4221.jpg}
        \caption{$0.14-4221$}
	\end{subfigure}
		\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/horse/x-4.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/horse/y-4-41-5276.jpg}
        \caption{$0.41-5276$}
	\end{subfigure}
		\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/horse/x-18.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/horse/y-18-55-20046.jpg}
        \caption{$0.55-20046$}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/horse/x-46.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/horse/y-46-66-49586.jpg}
        \caption{$0.66-49586$}
	\end{subfigure}
		\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/horse/x-85.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/horse/y-85-72-90731.jpg}
        \caption{$0.72-90731$}
	\end{subfigure}

	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/vangogh/0-x0.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_visuals/vangogh/0-y0.jpg}
        \caption{original}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/vangogh/x-4.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/vangogh/y-4-17-5276.jpg}
        \caption{$0.17-5276$}
	\end{subfigure}
		\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/vangogh/x-11.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/vangogh/y-11-35-12661.jpg}
        \caption{$0.35-12661$}
	\end{subfigure}
		\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/vangogh/x-19.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/vangogh/y-19-47-21101.jpg}
        \caption{$0.47-21101$}
	\end{subfigure}
	\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/vangogh/x-27.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/vangogh/y-27-68-29541.jpg}
        \caption{$0.68-29541$}
	\end{subfigure}
		\begin{subfigure}{.16\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/vangogh/x-89.jpg}
        \includegraphics[width=.98\linewidth]{theimgs/app_final_process/vangogh/y-89-82-94951.jpg}
        \caption{$0.82-94951$}
	\end{subfigure}
    \caption{The illustrations of \modelNameShort applied to the nullifying attack process on \textsc{black2blond}, \textsc{horse2zebra} and \textsc{photo2paint}.}
	\label{fig:process-null}
    \end{figure*}
    


==> thefigs/app_final_visuals/horse.tex <==
\begin{figure*}[t]
    \centering
    	\begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/11-x0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/13-x0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/15-x0.jpg}}{input}
    	\end{subfigure}
    	    \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/11-y0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/13-y0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/15-y0.jpg}}{expected}
    	\end{subfigure}
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/11-finalx.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/13-finalx.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/15-finalx.jpg}}{adversarial}
    	\end{subfigure}	
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/11-finaly.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/13-finaly.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/15-finaly.jpg}}{nullifying}
        \end{subfigure}
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/0-x0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/1-x0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/18-x0.jpg}}{input}
    	\end{subfigure}
    	    \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/0-y0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/1-y0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/18-y0.jpg}}{expected}
    	\end{subfigure}
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/0-finalx.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/1-finalx.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/18-finalx.jpg}}{adversarial}
    	\end{subfigure}	
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/0-finaly.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/1-finaly.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/horse/18-finaly.jpg}}{nullifying}
        \end{subfigure}
    \caption{Qualitative results of \modelNameShort against \textsc{horse2zebra} under the nullifying attack scheme. Although in some cases insignificant stripe-like patterns remain on the adversarial results (the ``nullifying'' columns), when compared to the expected results (the ``expected'' columns), the adversarial results are clearly closer to the input horse pictures than to the transformed zebra images.}
    \label{fig:horse}
    \end{figure*}

==> thefigs/app_final_visuals/label2facade.tex <==
\begin{figure*}[t]
    \centering
    	\begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/4-x0.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/5-x0.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/8-x0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/10-x0.jpg}}{input}
    	\end{subfigure}
    	    \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/4-y0.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/5-y0.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/8-y0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/10-y0.jpg}}{expected}
    	\end{subfigure}
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/4-finalx.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/5-finalx.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/8-finalx.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/10-finalx.jpg}}{adversarial}
    	\end{subfigure}	
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/4-finaly.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/5-finaly.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/8-finaly.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/10-finaly.jpg}}{distorting}
        \end{subfigure}
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/1-x0.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/2-x0.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/9-x0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/3-x0.jpg}}{input}
    	\end{subfigure}
    	    \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/1-y0.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/2-y0.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/9-y0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/3-y0.jpg}}{expected}
    	\end{subfigure}
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/1-finalx.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/2-finalx.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/9-finalx.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/3-finalx.jpg}}{adversarial}
    	\end{subfigure}	
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/1-finaly.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/2-finaly.jpg}
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/9-finaly.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/lab2face/3-finaly.jpg}}{distorting}
        \end{subfigure}
    \caption{Qualitative results of \modelNameShort against \textsc{label2facade} under the distorting attack scheme. In the ``expected'' columns, \textsc{label2facade} works as expected and produces realistic images of facades according to the input label maps. Similar to Figure \ref{fig:night2day}, when given adversarial images crafted by \modelNameShort, \textsc{label2facade} produces figures obscured by black and white blobs.}
    \label{fig:laba2facade}
\end{figure*}

==> thefigs/app_final_visuals/scm.tex <==
\begin{figure*}[t]
    \centering
	\begin{subfigure}{.12\linewidth}
        \centering
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/57-x0.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/58-ax0.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/7-ax0.jpg}
        \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/77-ax0.jpg}}{input}
	\end{subfigure}
	    \begin{subfigure}{.12\linewidth}
        \centering
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/57-y0.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/58-by0.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/7-by0.jpg}
        \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/77-by0.jpg}}{expected}
	\end{subfigure}
    \begin{subfigure}{.12\linewidth}
        \centering
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/57-finalx.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/58-finalx.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/7-finalx.jpg}
        \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/77-finalx.jpg}}{adversarial}
	\end{subfigure}	
    \begin{subfigure}{.12\linewidth}
        \centering
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/57-finaly.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/58-mine.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/7-mine.jpg}
        \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/77-mine.jpg}}{distorting}
    \end{subfigure}
    \begin{subfigure}{.12\linewidth}
        \centering
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/70-x0.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/17-ax0.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/23-ax0.jpg}
        \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/33-ax0.jpg}}{input}
	\end{subfigure}
	    \begin{subfigure}{.12\linewidth}
        \centering
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/70-y0.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/17-by0.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/23-by0.jpg}
        \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/33-by0.jpg}}{expected}
	\end{subfigure}
    \begin{subfigure}{.12\linewidth}
        \centering
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/70-finalx.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/17-finalx.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/23-finalx.jpg}
        \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/33-finalx.jpg}}{adversarial}
	\end{subfigure}	
    \begin{subfigure}{.12\linewidth}
        \centering
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/70-finaly.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/17-mine.jpg}
        \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/23-mine.jpg}
        \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/scm/33-mine.jpg}}{distorting}
    \end{subfigure}
    \caption{Qualitative results of \modelNameShort against \textsc{str2seg-mapillery} under the distorting attack scheme. Similar to the results of \textsc{str2seg} (Figure \ref{fig:str2seg-start}), the expected color patterns are 
    distorted. Irregular patterns of green, blue, light pink, and gray (representing trees, vehicles, sidewalk, and buildings) appear on road areas of the ``distorting'' results.}
    \label{fig:scm}
\end{figure*}

==> thefigs/app_final_visuals/vangogh.tex <==
\begin{figure*}[t]
    \centering
    	\begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/0-x0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/9-x0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/12-x0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/3-x0.jpg}}{input}
    	\end{subfigure}
    	    \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/0-y0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/9-y0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/12-y0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/3-y0.jpg}}{expected}
    	\end{subfigure}
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/0-finalx.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/9-finalx.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/12-finalx.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/3-finalx.jpg}}{adversarial}
    	\end{subfigure}	
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/0-finaly.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/9-finaly.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/12-finaly.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/3-finaly.jpg}}{nullifying}
        \end{subfigure}
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/2-x0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/3-x0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/4-x0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/4-x0.jpg}}{input}
    	\end{subfigure}
    	    \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/2-y0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/3-y0.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/4-y0.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/4-y0.jpg}}{expected}
    	\end{subfigure}
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/2-finalx.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/3-finalx.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/4-finalx.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/4-finalx.jpg}}{adversarial}
    	\end{subfigure}	
        \begin{subfigure}{.12\linewidth}
            \centering
            \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/2-finaly.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/3-finaly.jpg}
            % \includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/4-finaly.jpg}
            \stackunder[5pt]{\includegraphics[width=0.98\linewidth]{theimgs/app_final_visuals/vangogh/4-finaly.jpg}}{nullifying}
        \end{subfigure}
    \caption{Qualitative results of \modelNameShort against \textsc{photo2paint} under the nullifying attack scheme. Similar to the results of \textsc{horse2zebra} (Figure \ref{fig:horse}), although minor painting texture (with the style of Vincent van Gogh) can be found, the overall color scheme of the ``nullifying'' results is returned to that of the original ``input'' photos. Thus, the ``nullifying'' results are more similar to the ``input'' photos than to the ``expected'' results.}
    \label{fig:van-end}
    \end{figure*}



==> thefigs/exp_qualitative.tex <==

\begin{figure*}[t]\small
    \centering
    	\begin{subfigure}{.135\linewidth}
            \centering
    		\includegraphics[width=0.99\linewidth]{theimgs/qualitative/distorting/str_x0.jpg}
            \caption{{\scriptsize input}}
    	\end{subfigure}
    	    \begin{subfigure}{.135\linewidth}
            \centering
    		\includegraphics[width=0.99\linewidth]{theimgs/qualitative/distorting/str_y0.jpg}
            \caption{{\scriptsize expected}}
    	\end{subfigure}
        \begin{subfigure}{.135\linewidth}
            \centering
    		\includegraphics[width=0.99\linewidth]{theimgs/qualitative/distorting/str_yf.jpg}
    		\caption{{\scriptsize \modelNameShort}}
    	\end{subfigure}
	    \begin{subfigure}{.135\linewidth}
            \centering
            \includegraphics[width=0.99\linewidth]{theimgs/qualitative/distorting/str2seg_rgf.jpg}
		    \caption{{\scriptsize RGF}}
    	\end{subfigure}
        \begin{subfigure}{.135\linewidth}
            \centering 
            \includegraphics[width=0.99\linewidth]{theimgs/qualitative/distorting/str2seg_prgf.jpg}
            \caption{{\scriptsize PRGF}}
    	\end{subfigure}
	    \begin{subfigure}{.135\linewidth}
            \centering
            \includegraphics[width=0.99\linewidth]{theimgs/qualitative/distorting/str2seg_bandit.jpg}
            \caption{{\scriptsize Bandit}}
    	\end{subfigure}
        \begin{subfigure}{.135\linewidth}
            \centering
            \includegraphics[width=0.99\linewidth]{theimgs/qualitative/distorting/str2seg_zoom.jpg}
            \caption{{\scriptsize AutoZOOM}}
    	\end{subfigure}	
        \caption{The distorting attack in \textsc{street2segment}, \textsc{facade2label} and \textsc{label2facade}.}
        \label{fig:distorting}
        \vspace{-4mm}
\end{figure*}


==> thefigs/showcase_both.tex <==
\begin{figure}[t!]
    \centering
    	\begin{subfigure}{.24\linewidth}
            \centering
            \includegraphics[width=0.99\linewidth]{theimgs/showcase/blond_x0.jpg}
            \includegraphics[width=0.99\linewidth]{theimgs/showcase/6-x0.jpg}
    		\stackunder[5pt]{\includegraphics[width=0.99\linewidth]{theimgs/showcase/63-x0.jpg}}{input}
    	\end{subfigure}
    	    \begin{subfigure}{.24\linewidth}
            \centering
            \includegraphics[width=0.99\linewidth]{theimgs/showcase/blond_y0.jpg}
            \includegraphics[width=0.99\linewidth]{theimgs/showcase/6-y0.jpg}
    		\stackunder[5pt]{\includegraphics[width=0.99\linewidth]{theimgs/showcase/63-y0.jpg}}{expected}
    	\end{subfigure}
    	\begin{subfigure}{.24\linewidth}
            \centering
            \includegraphics[width=0.99\linewidth]{theimgs/showcase/blond_x_f.jpg}
            \includegraphics[width=0.99\linewidth]{theimgs/showcase/6-finalx.jpg}
    	    \stackunder[5pt]{\includegraphics[width=0.99\linewidth]{theimgs/showcase/63-finalx.jpg}}{adversarial}
    	\end{subfigure}
        \begin{subfigure}{.24\linewidth}
            \centering
            \includegraphics[width=0.99\linewidth]{theimgs/showcase/blond_y_f.jpg}
            \includegraphics[width=0.99\linewidth]{theimgs/showcase/6-finaly.jpg}
    		\stackunder[5pt]{\includegraphics[width=0.99\linewidth]{theimgs/showcase/63-finaly.jpg}}{result}
    	\end{subfigure}
    \caption{Examples of the nullifying attack against Img2Img GANs, \ie, \textsc{black2blond},  \textsc{none2glasses}, and \textsc{blue2red}. Images in the columns from left to right are the original input, \jy{the original model output}, the adversarial example, and \jy{the final model output given the adversarial example}. The adversarial example is constructed to be nearly identical to the original input.}
    \label{fig:scheme}
    \vspace{-2mm}
    \end{figure}
